Toward Realistic Adversarial Attacks in IDS: A Novel Feasibility Metric for Transferability

Transferability-based adversarial attacks exploit the ability of adversarial examples, crafted to deceive a specific source Intrusion Detection System (IDS) model, to also mislead a target IDS model without requiring access to the training data or any internal model parameters. These attacks exploit common vulnerabilities in machine learning models to bypass security measures and compromise systems. Although the transferability concept has been widely studied, its practical feasibility remains limited due to assumptions of high similarity between source and target models. This paper analyzes the core factors that contribute to transferability, including feature alignment, model architectural similarity, and overlap in the data distributions that each IDS examines. We propose a novel metric, the Transferability Feasibility Score (TFS), to assess the feasibility and reliability of such attacks based on these factors. Through experimental evidence, we demonstrate that TFS and actual attack success rates are highly correlated, addressing the gap between theoretical understanding and real-world impact. Our findings provide needed guidance for designing more realistic transferable adversarial attacks, developing robust defenses, and ultimately improving the security of machine learning-based IDS in critical systems.

==> macros.tex <==
% Configure a directory location for sections
\newcommand*{\sectiondir}{sections/}

% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output

\newcommand{\lvm}[1]{{\color{teal} LVM: #1}}
\newcommand{\se}[1]{{\color{blue} SE: #1}}
\newcommand{\eb}[1]{{\color{cyan} EB: #1}}

